The penumbra of open source: projects outside of centralized platforms are longer maintained, more academic and more collaborative

GitHub has become the central online platform for much of open source, hosting most open source code repositories. With this popularity, the public digital traces of GitHub are now a valuable means to study teamwork and collaboration. In many ways, however, GitHub is a convenience sample, and may not be representative of open source development off the platform. Here we develop a novel, extensive sample of public open source project repositories outside of centralized platforms. We characterized these projects along a number of dimensions, and compare to a time-matched sample of corresponding GitHub projects. Our sample projects tend to have more collaborators, are maintained for longer periods, and tend to be more focused on academic and scientific problems.

==> figure-academic.tex <==
\begin{figure}%
    \centering
    \includegraphics[width=0.98\linewidth]{figs/Trujillo2021_Figure6.pdf}
    \caption{
    \textbf{Comparing academic and non-academic Penumbra repositories to GitHub}
    %
Fifteen percent of Penumbra hosts are ``academic" under our definition, representing 37\% of all Penumbra repositories.
We find that academic repositories are maintained for about as long as non-academic Penumbra repositories, so academic development practices do not drive the divergence from GitHub development patterns that we observe.
Academic repositories have fewer editors per file than non-academic Penumbra repositories, however, more closely matching development practices seen on GitHub.
This refutes the hypothesis that the Penumbra differs widely from GitHub primarily due to academic influence.
}
    \label{fig:ac-non-ac-breakdown}
\end{figure}



==> figure-collaborating.tex <==
\begin{figure}[t!]
    %
    \centering
    \includegraphics[width=0.98\linewidth]{figs/Trujillo2021_Figure2.pdf}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_commits}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_contributors}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_files}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_editor_density}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_branches}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_message_lengths}
    \end{subfigure}
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    \caption{%
    \textbf{Editing and collaborating in the Penumbra and GitHub.}
    Comparison of GitHub and Penumbra samples on a variety of metrics. 
    %
    Unique users for all plots are determined by unique email addresses in commit data. File counts are taken at the HEAD commit of the main branch. Editor overlap is defined as average number of unique contributors that have edited each file. Panel (e) excludes two GitHub repositories with 500 and 1300 branches, to make trend comparison easier.
    %
    }
    \label{fig:github_comparison_no_time}
\end{figure}



==> figure-features.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\textwidth]{figs/permutation-importance-random-forest.pdf}
\caption{\textbf{Random forest model to delineate Penumbra and GitHub samples.}
Feature permutation importance (\cref{subsec:methods:statisticalmodels}) once nonlinear random forest regressions were trained to predict whether a project was on GitHub or in the Penumbra. 
The predictive performance is shown in the inset using an ROC curve of true positive rate (TPR) and false positive rate (FPR).
\label{fig:feature-importance-random-forest}
}
\end{figure}




==> figure-languages.tex <==
\begin{figure}[t]%
    \centering
    \includegraphics[width=0.98\linewidth]{figs/Trujillo2021_Figure4.pdf}
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    \caption{
    \textbf{Dominant language domains in the Penumbra and GitHub}
    Comparison of language popularity, measured by lines of code (LOC) in panels (a-b) and by file count in panels (c-d). We count the top languages of each repository by the specified metric, normalize the results to a percentage of independent or GitHub repositories, then subtract the percentages. Therefore a language with a value of $-0.05$, for example, is the top language on $5\%$ more GitHub repositories than Penumbra repositories, while a positive value indicates $5\%$ more Penumbra repositories than GitHub repositories.
    }
    \label{fig:lang}
\end{figure}   


==> figure-novelty.tex <==
\begin{figure}[h!]
    \centering
    %
    \includegraphics[width=0.8\linewidth]{figs/mirrors.pdf}
    \caption{\textbf{The Penumbra's intersection with other datasets.}
    Of the 55343 discovered, non-empty repositories,
    18\% have a first commit hash that can also be found on GitHub (GitHub Duplicate), but 30\% of those repositories diverge and contain code not found on GitHub (GitHub Diverged). Likewise, 7\% of Penumbra repositories have a first commit archived by Software Heritage~\cite{abramatic2018building}, and 14\% of those contain code not archived by Software Heritage. Finally, 21\% of Penumbra repositories share a commit with one or more other Penumbra repositories, and of these, 58\% have unique final commits.
    }
    \label{fig:mirrors}
\end{figure}



==> figure-overview.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figs/Trujillo2021_Figure1.pdf}
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    \caption{
    \textbf{The penumbra of open source.}
    (a) 
    Geographic distribution of hosts and unique email addresses (in parentheses) in our Penumbra sample.
    (b) 
    Distributions of emails per host and repositories per host.
    %
    (c) Distribution of unique emails per repositories.
    (d) Correlation between repositories and emails per host.
    We see that the number of repositories and email addresses generally correlate, with some outlying hosts with many more repositories than emails. 
    Academic hosts follow the same general trend, except that they tend to be larger than many non-academic hosts.
    (inset) Hosts are classified as ``academic" if over 50 percent of their email addresses end in \texttt{.edu} or come from a manually identified academic domain.
    }
    \label{fig:overview}
\end{figure}



==> figure-temporal.tex <==
\begin{figure}[t!]%
    \centering
    \includegraphics[width=0.98\linewidth]{figs/Trujillo2021_Figure3.pdf}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_age}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_age_over_comits}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_avg_interevent}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_burstiness}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_teamsize}
    \end{subfigure}
    \begin{subfigure}[b]{0\textwidth}
         \phantomcaption
         \label{fig:compare_dominance}
    \end{subfigure}
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    \caption{
    \textbf{Temporal characteristics of collaboration in the Penumbra and GitHub.}
    Comparison of GitHub and Penumbra samples on a variety of temporal metrics. The age of repository is given by the time between the first and latest commit. Panels (b-d) look at the heterogeneity of time between events. We first compare the distribution of mean interevent time to the distribution of ratios of age to number of commits, then show the distribution of index of dispersion per repository. Panels (e-f) compare how collaborative repositories actually are, or whether they are dominated by a single committer.
    }
    \label{fig:github_comparison_time}
\end{figure}



==> table-comparison.tex <==
%
\begin{table}
\caption{Comparison of Penumbra and GitHub datasets} %
\footnotesize
\makebox[\textwidth][c]{%
\begin{tabular}{llllllllll}
\toprule
\multicolumn{2}{c}{} & \multicolumn{3}{l}{Penumbra} & \multicolumn{3}{l}{GitHub} & \multicolumn{2}{l}{KS 2-Sample} \\
Statistic & Fig. & Mean & Median & CI & Mean & Median & CI & KS S & KS P \\ \midrule
Files & \ref{fig:github_comparison_no_time}(c) & 244.47 & 12 & [1,859] & 156.07 & 9 & [1,264] & 0.07 & $<$ 0.001 \\
Committers & \ref{fig:github_comparison_no_time}(b) & 2.39 & 1 & [1,6] & 2.08 & 1 & [1,3] & 0.17 & $<$ 0.001 \\
Message Lengths & \ref{fig:github_comparison_no_time}(f) & 29.24 & 20.80 & [7.00,67.33] & 24.23 & 17.60 & [7.42,56.00] & 0.13 & $<$ 0.001 \\
Editor Density & \ref{fig:github_comparison_no_time}(d) & 1.12 & 1.00 & [1.00,1.60] & 1.05 & 1.00 & [1.00,1.30] & 0.20 & $<$ 0.001 \\
Burstiness & \ref{fig:github_comparison_time}(d) & 4.86 & 2.88 & [0.50,14.51] & 3.68 & 2.15 & [0.17,11.24] & 0.13 & $<$ 0.001 \\
Commits & \ref{fig:github_comparison_no_time}(a) & 67.12 & 8 & [1,194] & 25.27 & 4 & [1,57] & 0.20 & $<$ 0.001 \\
Branches & \ref{fig:github_comparison_no_time}(e) & 1.74 & 1 & [1,4] & 1.67 & 1 & [1,5] & 0.03 & $<$ 0.001 \\
%
Age (hours) & \ref{fig:github_comparison_time}(a) & 5528 & 883 & [0.1,25556] & 2669 & 73 & [0.03,16194] & 0.26 & $<$ 0.001 \\
Age / Commits & \ref{fig:github_comparison_time}(b) & 283 & 39 & [0.02,1261] & 193 & 9 & [0.01,944] & 0.19 & $<$ 0.001 \\
Avg. Interevent & \ref{fig:github_comparison_time}(c) & 375 & 43 & [0.05,1547] & 257 & 11 & [0.02,1130] & 0.19 & $<$ 0.001 \\
Team Size & \ref{fig:github_comparison_time}(e) & 1.71 & 1.00 & [1.00,3.92] & 1.42 & 1.00 & [1.00,2.67] & 0.17 & $<$ 0.001 \\
\bottomrule
\end{tabular}}
\begin{flushleft}
\footnotesize
\medskip \par
%
Legend: Mean, median, and 5\textsuperscript{th} and 95\textsuperscript{th} percentile values from the Penumbra and GitHub samples for each statistic. \textbf{KS S} and \textbf{KS P} represent the Kolmogorov-Smirnov two-sample statistic, and its corresponding p-value. 
%
%
\end{flushleft}
\label{table:statistics_compared}
\end{table}

%



==> table-geographic.tex <==
\begin{table}%
\centering
%
\caption{Geographic split of our Penumbra (PN) and GitHub (GH)~\cite{2020octoverse} samples.}
\footnotesize
\makebox[\textwidth][c]{%
\begin{tabular}{rrrrrrr}\toprule
Region & \% Hosts & \% PN users & \% GH users~\cite{2020octoverse} & PN repositories (per capita) & \% Unique emails from academic domains \\ \midrule
EU &  39.35 & 73.47 & 26.8 & 83612 ($1.52 \times 10^{-4}$) & 39.20 \\
NA &  26.37 & 15.81 & 34 & 51245 ($2.97 \times 10^{-4}$) & 41.22 \\
AS &  30.95 &  7.38 & 30.7 & 21765 ($1.55 \times 10^{-5}$) & 1.21 \\
SA &   1.46 &  1.36 & 4.9 & 2776  ($1.64 \times 10^{-5}$) & 12.41 \\
OC &   1.60 &  1.93 & 1.7 & 3347  ($2.58 \times 10^{-4}$) & 65.24 \\
AF &   0.28 &  0.04 & 2 & 215   ($9.44 \times 10^{-7}$) & 0.00  \\ \bottomrule
\end{tabular}
\label{table:repos_per_continent}
}
\end{table}



==> table-logistic.tex <==
\newcommand{\pvalsmall}[0]{$< 0.001$}

\begin{table}[t]
    \centering
%
    \caption{Logistic regression models for GitHub vs. Penumbra outcome. 
    %
    %
    %
    %
    %
    \label{tab:logistics}
    }
%
\footnotesize
\makebox[\textwidth][c]{%
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{l}{Model 1} & \multicolumn{3}{l}{Model 2} \\
{} & $e^\beta$ &   $p$ &               CI & $e^\beta$ &   $p$ &             CI \\
\midrule
Constant                          &     0.188 & \pvalsmall{} &    [0.156,0.225] &     0.435 & \pvalsmall{} &  [0.364,0.520] \\
\textbf{Language} (vs.\ JavaScript)         &           &       &                  &           &       &                \\
\hspace{3mm} Bourne (Again) Shell &     3.478 & \pvalsmall{} &    [3.162,3.826] &           &       &                \\
\hspace{3mm} C                    &     4.065 & \pvalsmall{} &    [3.671,4.502] &           &       &                \\
\hspace{3mm} C\#                  &     1.589 & \pvalsmall{} &    [1.444,1.750] &           &       &                \\
\hspace{3mm} C++                  &     5.636 & \pvalsmall{} &    [5.184,6.127] &           &       &                \\
\hspace{3mm} C/C++ Header         &     5.829 & \pvalsmall{} &    [5.103,6.657] &           &       &                \\
\hspace{3mm} Java                 &     2.192 & \pvalsmall{} &    [2.070,2.321] &           &       &                \\
\hspace{3mm} Jupyter Notebook     &     2.722 & \pvalsmall{} &    [2.459,3.012] &           &       &                \\
\hspace{3mm} \textit{OTHER}       &     2.124 & \pvalsmall{} &    [2.023,2.230] &           &       &                \\
\hspace{3mm} PHP                  &     2.524 & \pvalsmall{} &    [2.323,2.743] &           &       &                \\
\hspace{3mm} Python               &     2.804 & \pvalsmall{} &    [2.651,2.965] &           &       &                \\
\hspace{3mm} TeX                  &    30.641 & \pvalsmall{} &  [25.348,37.040] &           &       &                \\
\hspace{3mm} TypeScript           &     1.078 & 0.187 &    [0.964,1.205] &           &       &                \\
\hspace{3mm} Vuejs Component      &     4.940 & \pvalsmall{} &    [4.331,5.635] &           &       &                \\
Files                             &     1.000 & \pvalsmall{} &    [1.000,1.000] &     1.000 & \pvalsmall{} &  [1.000,1.000] \\
Commits                           &     1.001 & \pvalsmall{} &    [1.001,1.001] &     1.001 & \pvalsmall{} &  [1.001,1.001] \\
Average editors per file          &     3.337 & \pvalsmall{} &    [3.002,3.709] &     3.328 & \pvalsmall{} &  [3.002,3.689] \\
Average message length            &     1.002 & \pvalsmall{} &    [1.001,1.002] &     1.002 & \pvalsmall{} &  [1.001,1.003] \\
Burstiness                        &     1.059 & \pvalsmall{} &    [1.055,1.063] &     1.058 & \pvalsmall{} &  [1.053,1.062] \\
Average interevent time [h]       &     1.000 & \pvalsmall{} &    [1.000,1.000] &     1.000 & \pvalsmall{} &  [1.000,1.000] \\
Branches                          &     0.971 & \pvalsmall{} &    [0.965,0.976] &     0.961 & \pvalsmall{} &  [0.955,0.966] \\
Lead workload                     &     0.461 & \pvalsmall{} &    [0.407,0.522] &     0.433 & \pvalsmall{} &  [0.384,0.489] \\
Committers                        &     0.945 & \pvalsmall{} &    [0.936,0.955] &     0.940 & \pvalsmall{} &  [0.931,0.950] \\
Effective team size               &     1.010 & 0.516 &    [0.980,1.040] &     1.016 & 0.315 &  [0.985,1.047] \\
-2LL                              & 84478.844 &       &                  & 89788.631 &       &                \\
Pseudo-R2                         &     0.100 &       &                  &     0.044 &       &                \\
\bottomrule
\end{tabular}
}
\end{table}



